Compositional Semantic Parsing Across Graphbanks

Most semantic parsers that map sentences to graph-based meaning representations are hand-designed for specific graphbanks. We present a compositional neural semantic parser which achieves, for the first time, competitive accuracies across a diverse range of graphbanks. Incorporating BERT embeddings and multi-task learning improves the accuracy further, setting new states of the art on DM, PAS, PSD, AMR 2015 and EDS.

==> pic-amr.tex <==

\captionsetup[sub]{font=small}

\begin{figure}
    \centering
    \begin{subfigure}{0.25\linewidth}
        \centering
	    \includegraphics[width=\linewidth]{pics/dot/amr}
		\caption{AMR}\label{fig:amr-am:amr}
	\end{subfigure}
	\begin{subfigure}{0.25\linewidth}
		\begin{center}
			\resizebox{\linewidth}{!}{
			\begin{forest}
				for tree={align=center}
				[{\app{\src{S}}}, for tree={fill=green!30}
					[{\app{\obj}}
						[{\G{want}}]
						[{\G{eat}}, for tree={fill=red!30}]
					]
					[{\modify{\src{M}}}, for tree={fill=brown!10!yellow!60}
						[{\G{cat}}]
						[{\G{shy}}, for tree={fill=blue!30}]
					]
				]
			\end{forest}}
		\end{center}
		\caption{AM term}\label{fig:amr-am:term}
	\end{subfigure}
		\begin{subfigure}{0.4\linewidth}
		\begin{center}
			\resizebox{\linewidth}{!}{
			\begin{forest}
				for tree={draw,align=center, no edge,l sep =0pt, l=\baselineskip}
				[parent, phantom
				[{$\bot$\\The}, name=the]
				[{\G{shy}\\shy}, name=shy, fill=blue!30]
				[{\G{cat}\\cat}, name=cat, fill=brown!10!yellow!60]
				[{\G{want}\\wants}, name=want, fill=green!30]
				[{$\bot$\\to}, name=to]
				[{\G{eat}\\eat}, name=eat, fill=red!30]
				]
				\draw[->] (want) to[out=north, in=80, edge node={node[above, fill=green!30] {\app{\src{S}}}}] (cat);
				\draw[->] (want) to[out=60, in=110, edge node={node[above, fill=green!30] {\app{\obj}}}] (eat);
				\draw[->] (cat) to[ out=100, in=north, edge node={node[above, fill=brown!10!yellow!60] {\modify{\src{M}}}}] (shy);%pos=0.65,
			\end{forest}}
		\end{center}
		\caption{AM dependency tree}\label{fig:amr-am:deptree}
	\end{subfigure}

	\begin{subfigure}{0.45\linewidth}
        \centering
	    \includegraphics[scale=0.28]{pics/dot/want}
	    \includegraphics[scale=0.28]{pics/dot/eat}
	    \includegraphics[scale=0.28]{pics/dot/cat}
	    \includegraphics[scale=0.28]{pics/dot/shy}
		\caption{\tiny Constants \G{want}, \G{eat}, \G{cat} and \G{shy}}\label{fig:amr-am:consts}
	\end{subfigure}\quad
	\begin{subfigure}{0.19\linewidth}
		\centering
		\includegraphics[scale=0.3]{pics/dot/wantEat}
		\caption{\tiny $\app{\src{O}}\of{\G{want},\G{eat}}$}\label{fig:amr-am:wantEat}
	\end{subfigure}$\:\:\:\:$
	\begin{subfigure}{0.2\linewidth}
		\centering
		\includegraphics[scale=0.3]{pics/dot/shyCat}
		\caption{\tiny $\modify{\src{M}}\of{\G{cat},\G{shy}}$}\label{fig:amr-am:shyCat}
	\end{subfigure}
\vspace{-6pt}
    \caption{AMR for \textit{The shy cat wants to eat} with its AM
      analysis. \todo{pixelly pics (also in fig 2)?}}
    \label{fig:amr-am}
\end{figure}

